ACR: A Benchmark for Automatic Cohort Retrieval

Identifying patient cohorts is fundamental to numerous healthcare tasks, including clinical trial recruitment and retrospective studies. Current cohort retrieval methods in healthcare organizations rely on automated queries of structured data combined with manual curation, which are time-consuming, labor-intensive, and often yield low-quality results. Recent advancements in large language models (LLMs) and information retrieval (IR) offer promising avenues to revolutionize these systems. Major challenges include managing extensive eligibility criteria and handling the longitudinal nature of unstructured Electronic Medical Records (EMRs) while ensuring that the solution remains cost-effective for real-world application. This paper introduces a new task, Automatic Cohort Retrieval (ACR), and evaluates the performance of LLMs and commercial, domain-specific neuro-symbolic approaches. We provide a benchmark task, a query dataset, an EMR dataset, and an evaluation framework. Our findings underscore the necessity for efficient, high-quality ACR systems capable of longitudinal reasoning across extensive patient databases.

==> 03.1-baselines.tex <==
\subsection{\method{} System Components}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Wael (Note to self): re-write this whole section

\begin{enumerate}
    \item Explain online vs offline processes 
    \begin{itemize}
        \item online vs offline processes
        \item index ideas: keyword index, vector db, knowledge base
        \item
    \end{itemize}

    \item Explain baselines in terms of the previous subsection

        \begin{itemize}
        \item passage retrieval: vdb
        \item iterative per-patient prediction
        \item Hypercube: Move the "knowledge representation" paragraph to the neuro symbolic
    \end{itemize}
    
    \item 
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In a typical information retrieval system\footnote{A query rewrite step and a reranking step can be employed to further improve the system, but they are out of scope of this study.}, an offline index is often created for faster retrieval. At interrogation time, the retriever takes in the query and matches it against the index to find eligible candidates. A reader can be employed to further reinforce the understanding of the patient’s medical record.

The longitudinal nature of EHRs presents unique challenges when it comes to building a cohort retrieval system that is accurate and reliable, which is a must-have requirement for healthcare applications.

\subsubsection{Offline Indexing}

Several approaches can be adopted for offline indexing of patient records, which can broadly be classified based on the level of information consolidation. Traditional sparse vector space models such as TF-IDF and BM25 offer partial knowledge compression by preserving lexical frequency information. Dense retrieval methods, on the other hand, can capture deeper semantic meanings and match documents to queries based on the overall context rather than just term overlap. However, the effectiveness of dense retrieval methods when handling long passages heavily depends on the granularity at which the corpus is segmented and indexed for inference. The choice of retrieval units can significantly impact dense retrieval methods' performance. For example, if the retrieval unit is too large (e.g., an entire document), the dense retriever may struggle to identify the most relevant sections within the document. On the other hand, if the retrieval unit is too small (e.g., a single sentence), the retriever may miss important context that spans multiple sentences or paragraphs. 
% Here, we explore three popular strategies for choosing the granularity of patient records, at chunk-level, at summary-level, and at symbolic level.
Here, we explore two popular strategies for choosing the granularity of patient records, at the chunk level and at the symbolic level.

\paragraph{Concatenation of chunks.}
This strategy involves breaking down the documents into smaller chunks, which can then be retrieved and concatenated by the retriever at interrogation time. This has the advantage of preserving all information for interrogation time. However, it might introduce false positives as it offers little consolidation regarding event progression and resolution of contradictions and ambiguities, rendering it less accurate than other methods.

\paragraph{Symbolic Knowledge Representation.}
This strategy involves structuring patient information into a knowledge graph, much like \cite{wong_scaling_2023}. However, unlike \cite{wong_scaling_2023}, we examine a neuro-symbolic system (Epistemus) that utilizes unstructured text rather than semi-structured data.

In Epistemus, each medical report is fed to a \textit{lossless} clinical NLU process that interprets both the explicit text content and its tacit implications at a document level and faithfully transforms it into a proprietary knowledge representation (KR). Epistemus utilizes a novel Dynamic Symbolic Memory as it examines all KR artifacts extracted from each report and cross-references them against the evolving journey in the dynamic memory. When new evidence aligns with current knowledge, the engine consolidates events and refines their facts, boosting their confidence scores. Conversely, if evidence conflicts, the engine scrutinizes all contradictory beliefs within the journey, leveraging multiple symbolic AI and ML resources to ascertain the most plausible beliefs, updating or amending the memory as necessary. The result is a comprehensive, consistent, and coherent symbolic journey where each belief is both justifiable and traceable to its originating text. A proprietary event-rooted knowledge base is developed to allow efficient and effective reasoning across millions of patients to answer clinical questions. 
One type of question supported by Epistemus is cohort retrieval to which we are limiting the evaluation in this study. 
Additionally, Epistemus ranks the results in the retrieved cohort and provides explanations for the inclusion of each patient; both tasks are outside the scope of this paper.

\subsubsection{Online Interrogation}
There are three possible schemes for matching queries and patients (TrialGPT, DistillLLM). The “query-to-patient” scheme matches one trial to a list of patients. The “patient-to-query” iterates each patient in the list upon arrival of a new query. A less common scheme is “patient-to-patient” matching, where known eligible patients are matched with other patients to find unknown eligible ones. In cohort retrieval, patient data is usually write-once and read many times, while a large amount of clinical queries arrive in real time. The “query-to-patient” scheme aligns well with how cohort retrieval operates and will be the main focus of this study. Nevertheless, the “query-to-patient” scheme might not give us insights into the best performance of the baselines if we ignore efficiency. Therefore, we also consider the “patient-to-query” scheme even though they are not practical for cohort retrieval.

\paragraph{Passage Retrieval (Query-to-Patient Matching).}
The query-to-patient matching tasks mimic typical cohort retrieval tasks such as identifying a population for a clinical trial or identifying a sample for a cohort study or quality improvement project. 
We consider the dense retrieval systems.
% We consider the sparse (TF-IDF, BM25) and dense (OpenAI, PubMedQA) retrieval systems. 
Given a clinical query q, a cohort retrieval system searches for relevant passages from an indexed corpus (Section 3). Here, we have the option to return all unique patients associated with the retrieved passages. Or, we can employ a reader that resolves the retrieved passages per patient into a yes/no answer as to whether that patient is eligible for the query. We employed several LLM (GPT-4, Llama v2, Mistral) as our readers. These LLMs have a limited context length so the number of retrieved passages being considered by the reader is limited. To address this issue, we can consolidate the passages per retrieved patient using the same technique in Section 3.2. Several works try to address this problem (RoPE, YaRN, Attn-Sink) but they require fine-tuning and are out of the scope of this study. 

% \textbf{Expert system.} Some authors of this paper develop an expert system for cohort retrieval based on symbolic reasoning. A proprietary event-rooted knowledge base is developed to allow efficient and effective reasoning across millions of patients to answer clinical questions. One type of question supported by Epistemus is cohort retrieval to which we are limiting the evaluation in this study. Additionally, Epistemus ranks the results in the retrieved cohort and provides explanations for the inclusion of each patient; both tasks are outside the scope of this paper. Epistemus features a symbolic query language, named SQuerL, allowing users to effectively express any question supported by the KR. The execution of SQuerL over the knowledge base for large-scale reasoning is mathematically provable. Alternatively, an LLM-based language user interface (LUI) is provided to translate natural language questions into SQuerL. 

\paragraph{Iterative Per-Patient Prediction (Patient-to-Query Matching).}
Patient-to-query matching mimics clinical tasks including ascertaining whether a specific patient is eligible for a clinical trial or satisfies a quality metric. We employ the same system components of the “query-to-patient” matching approach. Given a clinical query,  we go through the patient list one-by-one and retrieve the relevant passages. Here, we can classify the patient as eligible if there exists some relevant passages. We can also apply the reading and summarizing steps as 4.2 to classify the patient. 

% A cohort retrieval system comprises a retriever, and optionally a machine reader and summarizer. Sometimes an indexer is involved in preparing the text passages for faster retrieval. A query rewriter is also involved to reformulate the query for better retrieval, toward both accuracy and speed. There is also a reranker that focuses on fine-grained reordering of documents within the retrieved document set (cite Zhu). In this work, we focus solely on the performance and efficiency trade-off without these optimizations. Therefore, we mainly focus on the three main components: the retriever, the reader, and the summarizer.

% \subsubsection{Baselines}
% In this work, we evaluate the performance of a commercial product for ACR, Epistemus, against two state-of-the-art (SoTA) baselines. 
% The first baseline, Passage Retrieval, leverages LLM embedding and vector databases to facilitate efficient retrieval. 
% The second baseline, Per-Patient Prediction, requires querying an LLM for each patient to ascertain if they meet the given criteria. Although this approach is impractical for real-world applications, potentially scaling to millions of patients, it serves as a theoretical benchmark – or an oracle – to gauge the maximum capabilities of SoTA LLMs in clinical reasoning for the ACR task. Table ABC shows a comparison of the three systems in terms of the choices made for their components. 

\subsubsection{Neuro-Symbolic Baseline}
Epistemus pairs LLMs with symbolic reasoning 
    %TODO (cite our KDD paper in the camera ready, not now, keep it anonymous) 
    in the following components depicted in \figureref{fig:overview}: 
\begin{enumerate}
    \item \textbf{Text-based reasoning:} Each medical report is fed to a lossless clinical NLU process that interprets both the explicit text content and its tacit implications at a document level, and faithfully transforms it into a proprietary Knowledge Representation (KR).

    \item \textbf{Longitudinal reasoning:} Epistemus utilizes a novel Dynamic Symbolic Memory as it examines all KR artifacts extracted from each report and cross-references them against the evolving journey in the dynamic memory. When new evidence aligns with current knowledge, the engine consolidates events and refines their facts, boosting their confidence scores. Conversely, if evidence conflicts, the engine scrutinizes all contradictory beliefs within the journey, leveraging multiple symbolic AI and ML resources to ascertain the most plausible beliefs, updating or amending the memory as necessary. The result is a comprehensive, consistent, and coherent symbolic journey where each belief is both justifiable and traceable to its originating text.

    \item \textbf{Large-scale reasoning:} A proprietary event-rooted knowledge base is developed to allow efficient and effective reasoning across millions of patients to answer clinical questions. One type of question supported by Epistemus is cohort retrieval to which we are limiting the evaluation in this study. Additionally, Epistemus ranks the results in the retrieved cohort and provides explanations for the inclusion of each patient; both tasks are outside the scope of this paper. 

    \item \textbf{Interface:} Epistemus features a \textbf{\textit{symbolic query language}}, named SQuerL, allowing users to effectively express any question supported by the KR. The execution of SQuerL over the knowledge base for large-scale reasoning is mathematically provable. Alternatively, an LLM-based language user interface (LUI) is provided to translate natural language questions into SQuerL. 

    
\end{enumerate}

==> 04-experiments.tex <==
\section{Experimental Results}

\input{tables/main_results}

\paragraph{Implementation Details.}
% Model performance is evaluated across two schemes, the efficiency-oriented ``query-to-patient'' scheme and the accuracy-oriented ``patient-to-query'' scheme. 
We employ the best models and technologies available at the time of submission for the dense retrievers and the readers. 
\textbf{Retriever:} We consider the following text embeddings OpenAI, SBert, PubMed QA SNLI, BioBERT QA, and SNLI. All medical documents are stored in the Chroma vector database. To accommodate the limited context window size of the reader, all documents are split into chunks of $1K$ tokens with a $10\%$ token overlap.
\textbf{Reader:}
% We employ zero-shot LLMs as the readers. We consider GPT-3.5 (\texttt{gpt-3.5-turbo-instruct}) with $4K$ context window and GPT-4 (\texttt{gpt-4-turbo-preview}) with $128K$ context window. 
We use GPT-4 (\texttt{gpt-4-turbo-preview}) with $128K$ context window. 
% We consider a zero-shot prompt as shown in the appendix. 
To ensure consistency and repeatability in our experiments, we set the temperature parameter to $0$. In addition, we set the top $p$ value to $0.95$ to eliminate randomness in the model's response generation. 
%
% \paragraph{Summarization}
% Most current readers have restrictions on the input length. Before passing the candidate set of reports to the reader, we summarize the retrieved contents. Summarization can happen at the indexing phrase (query independent) and in between retrieve and read steps (query dependent). We use the same large language models in the reading comprehension step for summarization. 
%

\subsection{Proposed Evaluation Framework}{\color{gray}
When evaluating ACR systems, it is important to consider that not all cohorts, and queries, will be of equal difficulty or can be compared to one another. More explicitly, when considering accuracy metrics for queries that return only a few, or no, patients from the original distribution errors carry a different weight than for those that return many. Thus comparing or aggregating these scores together can lead to a misleading characterization of a system's abilities. Similarly, conceptual complexity of each query will impact an ACR system's ability to adequately retrieve the correct cohort, as it will strongly depend on a system's ability to interpret the criteria and compare it against its representation of each patient and their respective medical journey. Lastly, an ACR system should be coherent, meaning that the cohorts returned by related queries should agree logically on the membership of patients in each query. For the aforementioned reasons, our evaluation framework presents three methods for categorizing based on cohort size, expert-determined complexity, and inter-query coherence.
\paragraph{Support Conditioned Evaluation}:
Queries are organized into 4 cohort size categories: \textbf{Broad} queries (18 queries) where $n \geq 50$, \textbf{Narrow} queries (13 queries), returning  $ n \in [10, 50)$ patients, \textbf{Sparse} queries (40 queries), with $n \in [1, 9]$ patients retrieved, and \textbf{Empty} queries (42 queries), which return no patients at all, where $n$ represents the size of the cohort.

% To address the variability in conceptual complexity and categorize the queries along this axis, each query was rated in complexity by clinical domain experts. For each query the experts chose a category of \textbf{Hard} (19 queries), \textbf{Medium} (52 queries), \textbf{Low} (33 queries), and \textbf{Base} (6 queries). The base difficulty questions were considered a fundamental minimum of knowledge extraction; questions that a cohort retrieval system needs to be able to answer, due to the coverage and frequency of the related concepts. For the Hard, Medium, and Low difficulty, the ratings came from the experts' rating of the necessary levels of clinical knowledge necessary in order for a human to achieve a comparable query task.
\paragraph{Domain Complexity} To address the variability in question complexity, clinical research experts subjectively estimated difficulty based on prior experience with current standard processes. Estimates composite of the number and sequence of the logical operators; the number and kind of clinical observations required to identify the cohort; the degree of biomedical specialization involved in interpreting the question properly; and overall length of the question. As some concrete examples:
\begin{itemize}
    \item ``Find me patients with lung cancer" is considered a base case level of complexity as it involves one condition widely known to non-specialists
    \item "Low" complexity questions like, ``Find me patients with advanced NSCLC", implicitly involve multiple conditions (stage, histology, tumor type), but "advanced NSCLC" is frequent in medical text as a single concept, and a low degree of medical specialization is needed to understand the question. 
    \item ``Find me patients with HR+/Her2- breast cancer and a mutation in PIK3CA" involves four conditions not always co-located in medical text and the would require a moderate degree of biomedical specialization needed to interpret % biomarker-driven retrieval questions successfully.
    \item Queries with a significant length, number of conditions, nested logic, and specialization needed to understand the question like, ``Show me adult patients with locally advanced or metastatic solid tumor, multiple myeloma or B cell non-Hodgkin lymphoma, ECOG 0-2, no primary brain tumors or leptomeningeal metastases, and one of the following genomic alterations: RET, VEGFR1/2/3, KIT, PDGFR, RAF-1, BRAF mutations or amplifications" is considered a high complexity question
\end{itemize}
While model performance of each of the models did highly correlate with the subjective estimates, rigorous formulation of clinical query complexity was outside the scope of this work so these are provisional categorizations and welcome further refinement.
\paragraph{Set-Theoretic Consistency}
Queries used in this study can be related to one-another, by one of the following types of relationships: \textbf{Synonym} queries are two queries which share the same meaning, but use different language to express it. As an example, ``Patients taking \underline{Tagrisso}", and ``Patients with \underline{osimertinib}" refer to the same medication, using a brand name in one, and the generic in the latter. In \textbf{Parent-Child} queries, cohorts related to a parent query, such as ``breast cancer patients", must be a strict super-set of the child,  "breast cancer patients with carcinoma" for example. Finally, queries that are set-completions are referred to as \textbf{Complimentary}. These might include queries that are simply negated, or use ``except" and ``exactly" . As a concrete example, ``Breast cancer patients with carcinoma" and ``breast cancer patients without carcinoma" should set complete children of the parent ``Breast cancer patients". 

With regards to Support Conditioned and Domain Complexity evaluations, our work follows established prior work, leveraging \textit{macro} (P)recision, (R)ecall, and F1-score for broad and narrow queries \cite{wong_scaling_2023}. However, due to the sensitivity of these metrics for sparse and empty queries, as well as, a higher likelihood for hallucinations, \textit{micro} False Positive Rate (FPR) is reported in order to demonstrate when ACR systems correctly reject patients from cohort inclusion. Additional metrics regarding feasibility and cost, both monetary and temporal, are considered as an additional comparison.
% \subsubsection{Inter-Query Coherence}


Our results include an analysis of Inter-Query Coherence (IQC) which explores the aforementioned query relationships, to evaluate the coherence between the retrieved cohorts by each proposed ACR system.
% Wael (Note to Self): describe whole framework explaining the following
% \begin{enumerate}
%     \item Query categorization: by cohort size, by expert-determined complexity
    
%     \item metrics:
%     \begin{itemize}
%         \item quality (P/R/F1)
%         \item hallucinations (FPR)
%         \item feasibility (time and cost of online operations)
%     \end{itemize}
    
%     \item Set closure (come up with a metric): measure system's unpredictability as it makes contradictory decisions based on the query. 
%     \begin{itemize}
%         \item paraphrasing as in Tagrisso
%         \item Subsets for And/OR (intersect/union)
%         \item negation
%         \item exclusion (except)
%         \item exactly
%         \item comparison operators
%     \end{itemize}
% \end{enumerate}

% Similar to prior work, such as \citep{wong_scaling_2023}, we compare system output against the gold cohorts and report Precision, Recall, and F1 scores (P/R/F1 scores). 
% However, we categorize queries into 4 groups based on their gold support (the number of patients in their ground-truth cohort): 
%     a) \textbf{broad-scope queries} returning at least $5\%$ of the patient populations;
%     b) \textbf{narrow-scope queries} returning less than $5\%$ of the population but 10 or more patients;
%     c) \textbf{sparse-response queries} returning $1$ to $9$ patients; and
%     b) \textbf{no-match queries} returning no patients.
%     %
    
% We report the \emph{macro} scores for the first two groups averaging over the individual scores of each query. 
% Due to the sparse response in the third group, P/R/F1 scores per query become very sensitive to a single true positive (TP), false positive (FP), or false negative (FN), rendering them meaningless. Additionally, ACR systems sometimes retrieve no answers to such queries resulting in an undefined precision ($0 \div 0$).
%     To address these issues, we propose measuring the \emph{micro} scores for this group, which is identical to grouping them into one set of TP, FP, and FN counts to collect statistically meaningful gold support.
% Furthermore, No-match queries have an undefined recall and as a result both macro and micro scores are meaningless. 
%     However, it is essential to measure the system's tendencies to overproduce false positives.
% For this purpose, we propose the \emph{False Positive Rate} ($FPR = \frac{FP}{FP+TN}$) to measure hallucination tendencies, that is when the retrieval system tends to return too many results that give it a high recall at the cost of false positives. 
% While, in the first two groups, the F1 score penalizes the hallucination phenomena by combining precision and recall, FPR is the proposed metric for the last two groups.
%We report FPR scores on all subset of queries as the other metrics, and ones that returned empty cohorts. 
%FPR plays a particularly important role in gaining insights of the performance on the last two query groups, where other metrics are undefinable due to division by zero.
%
%queries that returned at least $5\%$ of the patient populations, and ones that returned more than 10 patients and less than $5\%$ of the patient populations. For queries with $1$ to $9$ returned patients, we report the \emph{micro} scores. 
% Due to the scale and the cost of annotation, some previous work resort to ranking metrics such as Normalized Discounted Cumulative Gain at rank k ($NDCG@k$) and Precision at rank k ($Pr@k$)  for evaluation. 
%In addition to standard metrics, we propose the \emph{False Positive Rate} ($FPR = \frac{FP}{FP+TN}$) to measure hallucination tendencies, that is, when the retrieval system tends to return too many results that give it a high recall at the cost of false positives. 
%We report FPR scores on all subset of queries as the other metrics, and ones that returned empty cohorts. 
%FPR plays a particularly important role in gaining insights of the performance on the later queries subset, where other metrics are undefinable due to division by zero.

\subsection{Overall Comparison}

\tableref{tab:main_results} shows the quality performance of cohort retrieval systems on precision oncology queries in the typical retrieval setting and in an ``oracle'' setting where the sizes of the gold cohorts are known. 
For brevity, the table reports the numbers on queries with significant retrieved cohort (at least $5\%$ of the patient populations), the rest of the numbers are reported in \appendixref{apd:results}. 
%
The neuro-symbolic model (\hc{}) performs well across all settings, 
    striking a good balance between precision and recall at 76.2\% and 87.4\%, respectively. 
%
Meanwhile, the retrieve-and-read model (ADA-GPT-4) achieves the best precision at 79.4\% (3.2\% higher than \hc{}), 
    but at the cost of filtering out more than half of the eligible patients (a recall of 47\%, 40\% lower than \hc{}).
%
The performance of the retrieve-only models is promising, especially without any fine-tuning of the embeddings  . 

\input{images/figure_f1_fpr_5percent}

Regarding the quality performance per individual queries, the \hc{} system consistently outperforms others across all queries (\figureref{fig:f1_fpr_5percent}). The FPR plot shows some interesting conjectures on the retrievers and readers. 
%
The OpenAI's retriever and reader are more conservative and tend to reject the retrieved documents than the rest of the systems. 
%
The neuro-symbolic system \hc{} has spikes in FPR for some queries, but consistently behaves well for the rest. 
%
Smaller scale retrievers tend to over-predict the eligible patients, suggesting that fine-tuning is required for better performance. 

% \subsection{Comprehensiveness of ACR systems}
% \paragraph{Paraphrases queries.}

\subsection{The Complexity of Queries }
We demonstrate that ACR performances match well with human experts' estimation of query complexity. As shown in \figureref{fig:complexity}, harder queries perform worse than easier ones. \hc{} performs well at all difficulty levels, except for base queries. The performances indicate that the set of test questions is well-crafted for the task by introducing queries that effectively measure the current systems while encouraging more require more efforts to solve the more challenging queries. 
% We demonstrate that the performances of ACR match well with human experts estimation of the query complexity. In , hard queries show lower performance, and vice versa. 

\input{images/figure_query_complexity_f1}

% Model ABC works well across multiple domain where model XYZ suffers. 

% How resilience are the models w.r.t the queries complexity?
}
